Purchase and Production Optimization in a Meat Processing Plant

The food production industry, especially the meat production sector, faces many challenges that have even escalated due to the recent outbreak of the energy crisis in the European Union. Therefore, efficient use of input materials is an essential aspect affecting the profit of such companies. This paper addresses an optimization problem concerning the purchase and subsequent material processing we solved for a meat processing company. Unlike the majority of existing papers, we do not concentrate on how this problem concerns supply chain management, but we focus purely on the production stage. The problem involves the concept of alternative ways of material processing, stock of material with different expiration dates, and extra constraints widely neglected in the current literature, namely, the minimum order quantity and the minimum percentage in alternatives. We prove that each of these two constraints makes the problem \mbox{$\mathcal{NP}$-hard}, and hence we design a simple iterative approach based on integer linear programming that allows us to solve real-life instances even using an open-source integer linear programming solver. Another advantage of this approach is that it mitigates numerical issues, caused by the extensive range of data values, we experienced with a commercial solver. The results obtained using real data from the meat processing company showed that our algorithm can find the optimum solution in a few seconds for all considered use cases.

==> Discussion.tex <==
The results published in this paper are based on a project with Sabris CZ, s.r.o., and it aims to develop a system for purchase and production planning in the meat processing company MÚÚÚ Písek.
In this section, we want to summarize a few observations from this close cooperation and provide insightful observations related to developing and deploying such a solution. The critical aspect of this project was an analysis of the needs of MÚÚÚ Písek and the revision of data. Namely, the revision of the data was the most demanding part of the project, but it is an essential step for MÚÚÚ Písek toward further digitization. To quantify this, less than 10\% of the effort in the project was dedicated to developing the algorithm. The rest was the problem analysis, data revision, and interconnection of the algorithm with the information system. Our aim in developing the algorithm was to avoid unnecessary expenses; therefore, we have developed the iterative constraint generation algorithm described in Section~\ref{sec:algorithm}. Its advantages are that (i) it does not require an expensive ILP solver, and (ii) it has a positive impact on the numerical stability of the ILP solver used inside the algorithm. Experiments with an open-source ILP solver confirmed that a commercial ILP solver is not needed. The experimental results have shown that the above-described ILP formulation is very fast. Nevertheless, concerning the complexity results provided in Section~\ref{sec:complexity}, there is no guarantee that it will also be fast for a different production or company. Therefore we do not purely count on the ILP formulation and propose to use the algorithm. In terms of solution quality, the preliminary analysis revealed that the solution provided by the algorithm is at least as good as the one constructed by planners. However, since the integration of the algorithm into the information system is still in progress and the weights used in the objective function need to be fine-tuned to the needs of MÚÚÚ Písek, we cannot quantify this at this moment. Nevertheless, planning with our algorithm is significantly faster compared to manual planning. Since our solution can be provided in seconds (including communication with the information system), it offers many advantages for planners. First, the planners can react quickly to changes in demand and compare several scenarios computed by the algorithm. This is not realistic when the plan is constructed manually. Another significant benefit for planners is that they can analyze the production process more. An example was illustrated in Section \ref{sec:numberOfHogs}, showing the relation between the number of hogs slaughtered and the optimal purchase and production plan cost. This analysis provides a closer view of the entire cost and the utilization of stock, stock turnover, materials shelf life, etc.
